Machine Learning-enhanced Receive Processing for MU-MIMO OFDM Systems

Machine learning (ML) can be used in various ways to improve multi-user multiple-input multiple-output (MU-MIMO) receive processing. Typical approaches either augment a single processing step, such as symbol detection, or replace multiple steps jointly by a single neural network (NN). These techniques demonstrate promising results but often assume perfect channel state information (CSI) or fail to satisfy the interpretability and scalability constraints imposed by practical systems. In this paper, we propose a new strategy which preserves the benefits of a conventional receiver, but enhances specific parts with ML components. The key idea is to exploit the orthogonal frequency-division multiplexing (OFDM) signal structure to improve both the demapping and the computation of the channel estimation error statistics. Evaluation results show that the proposed ML-enhanced receiver beats practical baselines on all considered scenarios, with significant gains at high speeds.

==> sections/HyperMIMO.tex <==
\section{HyperMIMO} 
\label{sec:HyperMIMO}



==> sections/background.tex <==
\section{Background} 
\label{sec:Background}


==> sections/problems.tex <==
\section{Problem statement} 
\label{sec:system_model}

We consider a \gls{MU-MIMO} system where $N_k$ single-antenna users transmit and receive to and from a base station equipped with $N_m$ antennas.
The number of bits sent per channel use by a transmitter is denoted $b$, and $\mathcal{C} = \LP c_1, \cdots, c_{2^b} \RP$ is the constellation of the corresponding \gls{QAM}.
In the following, we will introduce the channel model and detail the uplink and downlink setup, which comprise the channel estimation, equalization, and demapping of the received signal.

\subsection{Channel Model}
 
Each transmitter uses \gls{OFDM} to transmit on multiple subcarriers simultaneously. 
A group of $12$ adjacent subcarriers is called a \gls{RB}, and a transmission can span multiple \gls{RB}. 
The total number of used subcarriers is denoted $N_f$.
To study both the uplink and downlink scenario, we leverage a \gls{TDD} frame structure, where two consecutive time slots are used to separate the uplink and downlink transmissions. 
One slot comprises $N_t$ \gls{OFDM} adjacent symbols in time. We call \gls{RG} the grid comprising the $N_f$ subcarriers  and $2N_t$ symbols, and \gls{RE} one element in that grid. 
An example of resource grid is visible in the Figure \ref{fig:resource_grid}.
 

\begin{figure}[ht]
\centering
\begin{minipage}[b]{0.2\linewidth}
\includegraphics[height=150pt]{figs/resource_grid.png}
\caption{A resource grid.}
\label{fig:resource_grid}
\end{minipage}
\hspace{10pt}
\begin{minipage}[b]{0.75\linewidth}
\includegraphics[width=162pt]{figs/1_pilot.png} \hspace{5pt}
\includegraphics[width=162pt]{figs/2_pilots.png}
\caption{1- and 2-pilots patterns, where each number corresponds to a different transmitter.}
\label{fig:pilot_patterns}
\end{minipage}
\end{figure}

The channel is represented as a 4-dimensional tensor denoted by $\Hm \in \CC^{N_f \times 2N_t \times N_m \times N_k}$. 
Following the notations, $\Hm_{f, t} \in \CC^{N_m \times N_k}$ is the channel matrix at subcarrier $f$ and time $t$, and $\hv_{f, t, k}$ is the channel vector at subcarrier $f$ and time $t$ for the user $k$. 
It is important to note that the channel realizations corresponding to symbols $ t\in \LP 1, \dots,  N_t \RP$ are the ones seen in the uplink, while the realizations corresponding to symbols $ t\in \LP N_t+1, \dots, 2N_t \RP$ are seen in the downlink.
To estimate the channel, the transmitter(s) sends pilot symbols according to a 1- or 2-pilots pattern, which respectively contain pilots on one or two temporal positions within a slot. Figure \ref{fig:pilot_patterns} shows the 1- and 2-pilots patterns for 4 transmitters.
The set of pilot positions for a user $u$ is denoted $\mathcal{P}^{(u)}$ and the number of pilots in frequency and time are respectively denoted $N_{P_f}$ and $N_{P_t}$. For example, if a signal is transmitted on a single \gls{RB} using the 1-pilot pattern shown in Figure \ref{fig:pilot_patterns}, then $\mathcal{P}^{(1)} = \{\{1, 3\}, \{3, 3\}, \{5,3\}, \{7, 3\}, \{9, 3\}, \{11,3\}\}$, $N_{P_f} = 6$, and $N_{P_t} = 1$.
In the following, it is assumed that all pilots are orthogonal and do not interfere.
This can be achieved either by placing the pilots for each transmitter on different \gls{RE}, as visible in Figure~\ref{fig:pilot_patterns}, or by using Zadoff-Chu sequences.

\subsection{Uplink scenario}




In this first scenario, the base station aims to recover the bits sent simultaneously by the $k$ users on all \glspl{RE}. 
The tensors containing the the complex symbols send by the \glspl{UE} and received by the base station in the entire \gls{RG} are respectively denoted $\Xm \in \mathcal{C}^{N_f \times N_t \times N_m}$ and $\Ym \in \CC^{N_f \times N_t \times N_k}$.
$\xv_{f,t} \in \mathcal{C}^{N_k}$ and $\yv_{f,t} \in \CC^{N_m}$ are respectively the sent and received vector of complex symbols sent in a single \gls{RE}.
The channel transfer function for a subcarrier $f$ and a symbol $t$ is
\begin{equation}
\label{eq:transfert_function}
\yv_{f,t} = \Hm_{f,t} \xv_{f,t} + \nv_{f,t} \quad \ 1 \leq f \leq N_f, 1 \leq t \leq N_t,
\end{equation}
where $\nv_{f,t} \in \CC^{N_a}$ is the vector of complex \gls{AWGN} with variance $\sigma^2$ per element. For simplicity, we assume that the noise variance is constant over the \gls{RG}. 
The overall uplink architecture is illustrated in Figure \ref{fig:downlink}.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{figs/uplink.png}
    \caption{Uplink scenario.  $\widehat{\Xm}_1 \in \CC^{N_f \times N_t}$ and $\widehat{\Xm}_{N_k} \in \CC^{N_f \times N_t}$ are the demapped symbols for the user $1$ and $N_k$ respectively. }
    \label{fig:uplink}
\end{figure}

%\begin{itemize}
%	\item $\yv_{f,t} \in \CC^{N_a}$ is the vector of received complex symbols
%	\item $\Hm_{f,t} \in \CC^{N_a\times N_u}$ is the channel matrix
%	\item $\xv_{f,t} \in \mathcal{C}^{N_u}$ is the vector of sent complex symbols
%	\item $\mathcal{C} = \LP c_1, \cdots, c_{2^m} \RP$ is the constellation, $m$ being the number of bits sent per channel use.
%	\item $\nv_{f,t} \in \CC^{N_a}$ is the vector of gaussian noise
%	\item $f \in [1, N_{c}]$ denotes a subcarrier 
%	\item $t \in [1, N_{s}]$ denotes a symbol
%\end{itemize}

\subsubsection{Channel estimation}
\label{sec:ch_est_1}
As the received pilots symbols are assumed orthogonal, channel estimation can be carried out for each user in parallel. 
The optimal linear estimations of the channel at pilot positions is obtained by leveraging the \gls{LMMSE} estimator. If we denote $\Sigmam$ the channel covariance matrix at pilot positions, the channel estimates $\widehat{\Hm}_{\mathcal{P}^{(u)}} \in \CC^{N_{P_f} \times N_{P_t} \times N_m}$ for a user $u$ can be computed with
\begin{equation}
\text{vec}\LB\widehat{\Hm}_{\mathcal{P}^{(u)}}\RB = \Sigmam \LB \Sigmam  + \sigma^2 \RB^{-1} \text{vec}\LB\Ym_{\mathcal{P}^{(u)}}\RB,
\end{equation}
where $\Ym_{\mathcal{P}^{(u)}} \in \CC^{N_{P_f} \times N_{P_t} \times N_m}$ is the received signal at pilot positions.
We choose to perform the \gls{LMMSE} estimation at pilot position only since the channel covariance matrix is impossible to estimate precisely at data positions without resorting to costly measurement campaigns.
The channel estimation at any given position $\{f, t\}$ is assumed equal to the estimation obtained at the nearest pilot position  $\{\textrm{f}, \textrm{t}\} \in \mathcal{P}^{(u)}$, i.e., $\widehat{\Hm}_{f,t} = \widehat{\Hm}_{\{\textrm{f}, \textrm{t}\} \in \mathcal{P}^{(u)}}$.  
This is visible in Figure \ref{fig:pilot_patterns}, where dark lines delimits groups of \gls{RE} that shares the same channel estimates.
Please note that we are here only interested by the first $N_t$ symbols since we only estimate the uplink channel.
The overall estimated channel matrix is obtained by concatenating the channel estimates for each users and is denoted $\widehat{\Hm} \in \CC^{N_f \times 2N_t \times N_m \times N_k}$.
For a single \gls{RE}, we have 
\begin{equation}
\Hm_{f, t} = \widehat{\Hm}_{f, t} + \widetilde{\Hm}_{f, t} \quad \ 1 \leq f \leq N_f, 1 \leq t \leq 2N_t,
\end{equation}
where  $\widetilde{\Hm}_{f, t}$ is the channel matrix estimation error.
The sum of the channel estimation error covariances for all users  is denoted $\Em_{f,t} = \EE \LSB \widetilde{\Hm}_{f, t} \widetilde{\Hm}_{f, t}^H \RSB $.
%This quantity can be estimated following a similar process, starting with its computation for each user at pilot positions:
%\begin{equation}
%\Em^{(u)}_{\mathcal{P}^{(u)}} = \EE\LSB \text{vec}\LB \widetilde{\Hm}_{\mathcal{P}^{(u)}}\RB  \text{vec}\LB \widetilde{\Hm}_{\mathcal{P}^{(u)}}\RB^H \RSB
%= \Sigmam - \Sigmam \LB \Sigmam  + \sigma^2 \RB^{-1}\Sigmam.
%\end{equation}
%In the following, we will only need the spatial error covariance matrix. For a single pilot position $\{\textrm{f}, \textrm{t}\} \in \mathcal{P}^{(u)}$, it is denoted
%\begin{equation}
%\Em^{(u)}_{\{\textrm{f}, \textrm{t}\} \in \mathcal{P}^{(u)}} = \EE \LSB \widetilde{\hv}_{\{\textrm{f}, \textrm{t}\} \in \mathcal{P}^{(u)}} \widetilde{\hv}_{\{\textrm{f}, \textrm{t}\} \in \mathcal{P}^{(u)}}^H \RSB \quad \in  \CC^{N_m \times N_m}
%\end{equation}
%and lies on the diagonal of $\Em^{(u)}_{\mathcal{P}^{(u)}}$.
%Again, the spatial channel estimation error covariance at any given position $\{f, t,\}$  is assumed equal to the estimation obtained at the nearest pilot position  $\{\textrm{f}, \textrm{t}\} \in \mathcal{P}^{(u)}$, i.e., $\widehat{\Em}^{(u)}_{f,t} = \Em^{(u)}_{\{\textrm{f}, \textrm{t}\} \in \mathcal{P}^{(u)}}$. 
%The overall spatial channel estimation error covariance matrix at any position is obtained by summing the estimations for each user :
%\begin{equation}
%\widehat{\Em}_{f,t}
%= \sum_{u=1}^{N_k} \widehat{\Em}^{(u)}_{f,t} \quad \in \CC^{N_m \times N_m}
%\end{equation}


\subsubsection{Equalization}
To recover the sent symbols, a well known detector is the \gls{LMMSE} equalizer, which is usually considered of low complexity. 
However,  a standard implementation would require a matrix inversion to be computed for every \gls{RE}, wich would be of prohibitive complexity with any large \gls{MU-MIMO} setup. 
Therefore, we implemented a grouped-\gls{LMMSE} equalizer, where a single \gls{LMMSE} equalization matrix is computed and applied to a group of \glspl{RE} across multiple subcarriers $f \in [F_b, F_e]$ and symbols $t \in [T_b, T_e]$.
The optimal grouped-\gls{LMMSE} equalization matrix, as demonstrated in Appendix \ref{app:LMMSE}, is 
%
\begin{equation}
\label{eq:W}
\Wm_{f, t} = \LB \sum_{\textrm{f}=F_b}^{F_e} \sum_{\textrm{t}=T_b}^{T_e}  \widehat{\Hm}_{\textrm{f}, \textrm{t}}^H \RB \LB \sum_{\textrm{f}=F_b}^{F_e} \sum_{\textrm{t}=T_b}^{T_e} \LB \widehat{\Hm}_{\textrm{f}, \textrm{t}} \widehat{\Hm}_{\textrm{f}, \textrm{t}}^H + \Em_{\textrm{f},\textrm{t}} + \sigma^2 \Id \RB \RB^{-1},  F_b \leq f \leq F_e, T_b \leq t \leq T_e.
\end{equation}
%
From an estimation theory point of view, this \gls{LMMSE} detector can be viewed as biased since if all \glspl{UE} send a unique constellation point $c$, $\EE \LSB \Wm_{f,t} \yv_{f,t} \RSB \neq c$.
Indeed, while the estimation error averaged over all constellation points is zero-mean, the error for any given constellation points might be nonzero-mean.
An unbiased estimation can be obtained by computing a diagonal scaling matrix 
\begin{equation}
\Dm_{f, t} = \LB  \LB \Wm_{f,t} \hat{\Hm}_{f, t} \RB \odot \Id_{N_u} \RB^{-1}
\end{equation}
and computing
\begin{equation}
\hat{\xv}_{f, t} = \Dm_{f,t} \Wm_{f, t} \yv_{f,t}.
\end{equation}
%

\subsubsection{Demapping} 

Let's denote $\underline{\wv}_{f, t, k}^\top$ the $k^{\text{th}}$ line of the matrix $\Wm_{f, t}$. 
We also denote $\hv_{f, t, k}$ the channel vector of user $k$ and $\Hm_{f, t, -k}$ the channel of all other users. 
The \gls{MU-MIMO} uplink transmission can now be seen as $k$ equivalent \gls{AWGN} transmissions :
%
\begin{equation}
\hat{x}_{f, t, k}= x_{f, t, k} + \underbrace{\frac{\underline{\wv}_{f, t, k}^\top \LB \widehat{\Hm}_{f, t, -k} \xv_{f, t, -k} + \widetilde{\Hm}_{f, t} \xv_{f, t} +  \nv_{f, t} \RB}{\underline{\wv}_{f, t, k}^\top \widehat{\hv}_{f, t, k} }}_{z_{f, t, k}} , \quad  z_{f, t, k} \sim \mathcal{C}\mathcal{N} \LB 0, \nu_{f, t, k}^2 \RB ,
\end{equation}
%
where $z_{f, t, k}$ is assumed to be Gaussian distributed and includes both the channel estimation error, the interferences and the noise seen by user $k$.
%
%\begin{equation}
%\hat{x}_{f, t, k}= x_{f, t, k} + z_{f, t, k}, \quad \quad z_{f, t, k} \sim %\mathcal{C}\mathcal{N} \LB 0, \nu_{f, t, k}^2 \RB
%\end{equation}
%
Its noise variance is given by
\begin{equation}
\nu_{f, t, k}^2 = \EE\LSB z_{f, t, k}^* z_{f, t, k} \RSB = \frac{\underline{\wv}_{f, t, k}^H \LB\widehat{\Hm}_{f, t, -k} \widehat{\Hm}_{f, t, -k}^H + \Em_{f,t} + \sigma^2 \Id_{N_a} \RB \underline{\wv}_{f, t, k}}{\underline{\wv}_{f, t, k}^H \widehat{\hv}_{f, t, k} \widehat{\hv}_{f, t, k}^H \underline{\wv}_{f, t, k}} .
\end{equation} 
%
We now denote $\mathcal{C}_{i,0}$ and $\mathcal{C}_{i,1}$ the subsets of $\mathcal{C}$ which contain all symbols for which the $i^{\text{th}}$ bit is respectively 0 and 1.
The \glspl{LLR} for the $i^{\text{th}}$ bit for the user $k$ on the RE $\LP f, t \RP$  can finally be computed with :
\begin{equation}
\text{LLR}_{f, t, k}^{\text{UL}}(i) = \ln{\frac{
\sum_{c\in\mathcal{C}_{i,1}} \exp{  - \frac{1}{\nu_{f, t, k}^2} \| \hat{x}_{f, t, k} - c\|^2 }
}{
\sum_{c\in\mathcal{C}_{i,0}} \exp{  - \frac{1}{\nu_{f, t, k}^2} \| \hat{x}_{f, t, k} - c\|^2 }
} } .
\end{equation}


\subsection{Downlink}

In this second scenario, the base station aims to simultaneously transmit to the $k$ \glspl{UE} on all \glspl{RE}. 
Here, the symbols sent by the \gls{BS} need to be precoded prior to the transmission to mitigate interferences. 
We recall that the downlink transmission happens on the second slot, with $N_t+1 \leq t \leq 2N_t$. 
We denote $\Um \in \mathcal{C}^{N_f \times N_t \times N_k}$ and $\Sm \in \CC^{N_f \times N_t \times N_m}$ the tensors of complex symbols respectively before and after precoding on the entire \gls{RG}.
Again, we denote $\uv_{f,t} \in \mathcal{C}^{N_k}$ and $\sv_{f,t} \in \CC^{N_m}$ the corresponding vector of on a single \gls{RE}. 
We also denote $\Rm \in \mathcal{C}^{N_f \times N_t \times N_k}$ and $\rv_{f,t} \in \CC^{N_k}$ respectively the tensor of received complex symbols on the entire \gls{RG} and the corresponding vector on a single \gls{RE}. 
For a subcarrier $f$ and a symbol $t$, the channel transfer function is
\begin{equation}
\rv_{f,t} = \Hm_{f,t}^H \sv_{f,t} + \qv_{f,t}  \quad \ 1 \leq f \leq N_f, N_t+1 \leq t \leq 2N_t,
\end{equation}
where $\qv_{f,t} \in \CC^{N_k}$ is the vector of complex \gls{AWGN} noise seen by the $k$ users with variance $\sigma^2$ per element. 
For simplicity, it is assumed that the uplink and downlink noise variances are equal.
We chose to use $\Hm_{f,t}^H$ instead of $\Hm_{f,t}^\top$ in the downlink channel model to simplify the following expressions, but the results are equivalents.
The downlink transmission process is shown in Figure \ref{fig:downlink}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\textwidth]{figs/downlink.png}
    \caption{Downlink scenario. $\widehat{\Rm}_1\in \mathcal{C}^{N_f \times N_t}$ and $\widehat{\Rm}_{N_k}\in \mathcal{C}^{N_f \times N_t}$ represent the signal received by the user $1$ and $N_k$ respectively, while $\widehat{\Gm}_{1,1}\in \mathcal{C}^{N_f \times N_t}$ and $\widehat{\Gm}_{N_k, N_k}\in \mathcal{C}^{N_f \times N_t}$  denotes the equivalent channel estimated by the user $1$ and $N_k$ respectively.}
    \label{fig:downlink}
\end{figure}

\subsubsection{Channel estimation and precoding at the \gls{BS}}

To precode the sent symbols, the \gls{BS} need to estimate the downlink channel for symbols $t \in \LP N_t+1, \dots, 2N_t \RP$. 
Thanks to the \gls{TDD} structure, the downlink channel is estimated using the pilots sent in the previous uplink slot, as seen in Section \ref{sec:ch_est_1}. 
Similarly, and since no pilot is received by the \gls{BS} in the downlink slot, the downlink channel estimates are assumed to be equal to the estimation computed for the nearest uplink pilots, i.e., $\widehat{\Hm}_{f, N_t+1 \leq t \leq 2N_t} = \widehat{\Hm}_{f, N_t}$.
Due to the uplink/downlink duality, the downlink precoding matrix is given by $\Wm_{f,t}^H$, the expression of which can be found in Equation \ref{eq:W} \cite{viswanath2003sum}. 
In order to normalize the average energy per sent symbol, we compute a matrix 
%
\begin{equation}
\Nm_{f, t} = \LB \LB \Wm_{f,t}\Wm_{f,t}^H \RB \odot \Id_{N_k} \RB^{-1}
\end{equation}
%
and the precoded symbols can be written as 
%
\begin{equation}
\sv_{f,t}  = \Wm_{f, t}^H \Nm_{f,t} \uv_{f,t}.
\end{equation}
%
The channel transfer function is now
\begin{equation}
\rv_{f,t} = \underbrace{\Hm_{f,t}^H \Wm_{f, t}^H \Nm_{f,t}}_{\Gm_{f,t}} \uv_{f,t} + \qv_{f,t} ,
\end{equation}
where we call $\Gm_{f, t}  \in \CC^{N_u \times N_u}$ the equivalent downlink channel.

\subsubsection{Channel estimation at the \glspl{UE}}
Let's call $\underline{\gv}_{f, t, k} $ the $k^{\text{th}}$ line of the matrix $\Gm_{f, t}$. 
This correspond to the channel seen by the user $k$. This can be split between the principal channel seen by the user $g_{f, t, k}$ and the interfering channels $\underline{\gv}_{f, t, -k}$. 
Each user only estimate their respective principal channel $\hat{g}_{f, t, k}$ with an error $\widetilde{g}_{f, t, k}$ and error variance $ v_{f,t,k} = \EE\LSB \| \widetilde{g}_{f, t, k} \|_2^2 \RSB $.
The mean interference power for user $k$ is denoted $j_{f,t,k} = \EE\LSB  \underline{\gv}_{f, t, -k}^H \underline{\gv}_{f, t, -k} \RSB$.
Similarly to the uplink scenario, the \gls{BS} sends orthogonal pilots according to the 1- or 2-pilots pattern. 
Each \gls{UE} then computes the \gls{LMMSE} channel estimation its pilot positions, estimations are assumed equal for the neighbouring data positions.
As the estimation process for each user is similar to the one detailed in Section \ref{sec:ch_est_1}, albeit with a single receiving antenna, it will not be further detailed here.
The equivalent downlink channel covariance matrix, needed to compute both the channel estimates and the estimation error variance, is denoted $\Omegam$.
The tensor of estimated downlink equivalent channel on the entire \gls{RG} is called $\widehat{\Gm} \in \mathcal{C}^{N_f \times N_t \times N_k \times N_k}$, and is formed by the estimations on all \gls{RE}:
\begin{equation}
\widehat{\Gm}_{f, t} = \diag \LB \LSB \hat{g}_{f, t, 0}, \cdots, \hat{g}_{f, t, N_k} \RSB \RB \in \mathcal{C}^{N_k \times N_k}.
\end{equation}
It should be noted that $\widehat{\Gm}_{f, t}$ is a diagonal matrix, since the \glspl{UE} do not estimate the interferences.
%
Finally, the sent symbols can be recovered with
\begin{equation}
\hat{\uv}_{f, t} = \widehat{\Gm}_{f, t}^{-1}  \rv_{f, t} = \widehat{\Gm}_{f, t}^{-1} \LB \Gm_{f, t}  \uv_{f, t} + \qv_{f, t} \RB,
\end{equation}

\subsubsection{Demapping}

The \gls{MU-MIMO} downlink transmission can also be seen as $k$ equivalent \gls{AWGN} transmissions :

\begin{equation}
\hat{u}_{f, t, k}
= u_{f, t, k}
+\underbrace{\frac{ \widetilde{g}_{f, t, k} u_{f, t, k} 
+ \underline{\gv}_{f, t, -k}^\top \uv_{f, t, -k}
+ q_{f, t, k}}{\hat{g}_{f, t, k}}}_{v_{f, t, k}} 
 \quad \quad v_{f, t, k} \sim \mathcal{C}\mathcal{N} \LB 0, \tau_{f, t, k}^2 \RB ,
\end{equation}
where $v_{f, t, k}$ is assumed to be Gaussian distributed with noise variance
\begin{equation}
\tau_{f, t, k}^2
= \EE\LSB v_{f, t, k}^* v_{f, t, k} \RSB 
=\frac{\overbrace{\EE\LSB \| \widetilde{g}_{f, t, k} \|_2^2 \RSB }^{v_{f,t, k}} 
+ \overbrace{\EE\LSB  \underline{\gv}_{f, t, -k}^H \underline{\gv}_{f, t, -k} \RSB }^{j_{f,t, k}}
+ \sigma^2 }{\| \hat{g}_{f, t, k} \|_2^2} .
\end{equation}

The \glspl{LLR} for the $i^{\text{th}}$ bit for the user $k$ on the \gls{RE} $\LP f, t \RP$ is obtained with:

\begin{equation}
\text{LLR}_{f, t, k}^{\text{DL}}(i) = \ln{\frac{
\sum_{c\in\mathcal{C}_{i,1}} \exp{  - \frac{1}{\tau_{f, t, k}^2} \| \hat{u}_{f, t, k} - c\|^2 }
}{
\sum_{c\in\mathcal{C}_{i,0}} \exp{  - \frac{1}{\tau_{f, t, k}^2} \| \hat{u}_{f, t, k} - c\|^2 }
} } .
\end{equation}



